Hyper-Kamiokande Design Report

On the strength of a double Nobel prize winning experiment (Super)Kamiokande and an extremely successful long baseline neutrino programme, the third generation Water Cherenkov detector, Hyper-Kamiokande, is being developed by an international collaboration as a leading worldwide experiment based in Japan. The Hyper-Kamiokande detector will be hosted in the Tochibora mine, about 295 km away from the J-PARC proton accelerator research complex in Tokai, Japan. The currently existing accelerator will be steadily upgraded to reach a MW beam by the start of the experiment. A suite of near detectors will be vital to constrain the beam for neutrino oscillation measurements. A new cavern will be excavated at the Tochibora mine to host the detector. The experiment will be the largest underground water Cherenkov detector in the world and will be instrumented with new technology photosensors, faster and with higher quantum efficiency than the ones in Super-Kamiokande. The science that will be developed will be able to shape the future theoretical framework and generations of experiments. Hyper-Kamiokande will be able to measure with the highest precision the leptonic CP violation that could explain the baryon asymmetry in the Universe. The experiment also has a demonstrated excellent capability to search for proton decay, providing a significant improvement in discovery sensitivity over current searches for the proton lifetime. The atmospheric neutrinos will allow to determine the neutrino mass ordering and, together with the beam, able to precisely test the three-flavour neutrino oscillation paradigm and search for new phenomena. A strong astrophysical programme will be carried out at the experiment that will detect supernova neutrinos and will measure precisely solar neutrino oscillation.

==> design-summary/summary.tex <==
%---------------------------------------------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Summary of the Hyper-Kamiokande detector timeline}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\graphicspath{{design-summary/figures/}}

\begin{figure}[htbp]
  \begin{center}
  \includegraphics[width=1.0\textwidth]{HK_timeline_NamatameCheck_v2_Eng.pdf}
   \caption{Construction period for the \hksingletank{}}
  \label{fig:construction-perod-1TankHD}
  \end{center}
\end{figure}

Figure~\ref{fig:construction-perod-1TankHD} shows the estimated construction
period of the Hyper-K detector for \hksingletank{}.
The construction is estimated to take about 10 years 
including the geological survey and final design making.


For the operation of the \hksingletank{} detector, 
necessary manpower is estimated to be
about 20 full-time equivalent (FTE) by taking into account
management and detector calibration
in addition to the operation and maintenance of water system, electronics,
DAQ system, and computer system. 
In the case of three tank case, the necessary FTE would be as twice as
the single tank case.


==> natbib/README <==
                                 What is NATBIB?
                                 
It is a LaTeX (2e, with some support for 2.09) package to act as generalized
interface for standard and non-standard bibliographic style files (BibTeX).

It is intended primarily to produce author-year style citations from a variety
of non-standard .bst outputs; it therefore replaces the special and individual
packages that go along with such .bst files:
   apalike.sty    for    apalike.bst et al.
   newapa.sty            newapa.bst, 
   chicago.sty           chicago.bst, named.bst et al.
   harvard.sty           agsm.bst, dcu.bst, kluwer.bst et al.
   astron.sty            astron.bst, apa.bst, humanbio.bst, et al.
   authordate<n>.sty     authordate<n>.bst, aaai-named.bst
   
The above .bst files may also be used with natbib to produce author-year or 
numerical citations, so that switching from author-year to numerical is only 
a matter of selecting an option. 

The standard .bst files (plain et al) and other numerical citation .bst files
are also understood, but they can produce only numerical citations.
Replacement .bst files
   plainnat.bst
   abbrvnat.bst
   unsrtnat.bst
are provided to produce the same formatting of the reference list as the
standard equivalent, but allowing both author-year and numerical citations.

See my parallel custom-bib system for generating customized bst files.

For installation instructions and more details, see README.vxx.

Patrick W. Daly
Max-Planck-Institut f\"ur Sonnensystemforschung
D-37191 Katlenburg-Lindau, Germany
E-mail: daly@mps.mpg.de

